40 Years of Calculus in 4 + epsilon Dimensions

Modern physics describes elementary particles by a formalism known as Quantum Field Theory. However, straight calculations with this formalism lead to numerous divergences, hence one needs a suitable regularization scheme. 40 years ago a surprising scheme was established for this purpose: Dimensional Regularization. One computes in "4 + epsilon space-time dimensions", and takes the limit to our 4 dimensional space-time at the end. This method caused a revolution in particle physics, which led to the Standard Model. Many people refer to its results, and even apply it, without being aware that its history actually started in Latin America, more precisely in La Plata, Argentina. ----- La f\'isica moderna describe a las part\'iculas elementales por medio del formalismo conocido como Teor\'ia Cu\'antica de Campos. Sin embargo, los c\'alculos directos realizados con este formalismo llevan a una gran cantidad de divergencias, por lo que es necesario un m\'etodo para regularizarlos. Hace 40 a\~nos se estableci\'o un esquema sorprendente para este objetivo: la Regularizaci\'on Dimensional. Se calcula en "4 + epsilon dimensiones espacio-temporales", y al final se toma el l\'imite a nuestro espacio y tiempo en 4 dimensiones. Este m\'etodo caus\'o una revoluci\'on en la f\'isica de part\'iculas, que result\'o en el Modelo Est\'andar. Muchas personas hacen referencia sus resultados, e incluso la aplican, sin saber que su historia comenz\'o en Am\'erica Latina, precisamente en La Plata, Argentina.

==> refsbolE.tex <==
\begin{thebibliography}{10}

\bibitem{SM} L.\ Glashow,
%Partial-symmetries of weak interactions
{\it Nucl.\ Phys.}\ {\bf 22} (1961) 579-588. 
S.\ Weinberg,
%A Model of Leptons
{\it Phys.\ Rev.\ Lett.}\ {\bf 19} (1967) 1264-1266. 
A.\ Salam,     
%Weak and electromagnetic interactions, 
en {\it Proc.\ of the 8th Nobel Symposium on} ``Elementary particle 
theory, relativistic groups and analyticity'', 
ed.\ N.\ Svartholm (1969) p.\ 367-377.

\bibitem{tHooft71} G.\ 't Hooft,	
%Renormalization of Massless Yang-Mills Fields
{\em Nucl.\ Phys.}\ {\bf B33} (1971) 173-199;
%Renormalizable Lagrangians for Massive Yang-Mills Fields
{\em Nucl.\ Phys.}\ {\bf B35} (1971) 167-188.

\bibitem{GelShi} I.M.\ Gel'fand y G.E.\ Shilov,
``Generalized Functions, volume 1: Properties and Operations'', 
Academic Press, New York (1964).

\bibitem{anareg} C.G.\ Bollini, J.J. Giambiagi y A.\
Gonz\'{a}les Dom\'{\i}nguez, 
%Analytic Regularization and the Divergences of Quantum Field Theories, 
{\it Nuovo Cim.}\ {\bf 31} (1964) 550-561.
 	
\bibitem{Speer72} E.R.\ Speer,
%On the structure of analytic renormalization.
{\it Commun.\ Math.\ Phys.}\ {\bf 23} (1971) 23-36. 
%, Erratum-ibid. 25 (1972) 336

\bibitem{bio} D.\ Bes, ``Juan Jos\'{e} Giambiagi'' en Conferencia
``La F\'{\i}sica del Siglo XX a Vuelo de P\'{a}jaro'',
Universidad de Buenos Aires (1996).
%www.df.uba.ar/index.php?option=com$\_$content&view=article&id=6613:juan-jose-giambiagi&catid=48&Itemid=196
F.A.\ Schaposnik,
``Un f\'{\i}sico argentino'', Art\'{\i}culo en memoria de 
J.J.\ Giambiag, {\it Perfis}, eds.\ F.\ Caruso y A.\ Troper, 
CBPF-CNPq, Brasil, 1997;
``Sobre el Premio Nobel de F\'{\i}sica 1999'',
{\it Ciencia Hoy} {\bf 10} No.\ 55 (2000).
%sites.google.com/site/schaposnik/sobreelpremionobeldefísica1999.
%Centro Brasileiro de Pesquisas F\'{\i}sicas (1996).

\bibitem{NC72} C.G.\ Bollini y J.J. Giambiagi, 
%Dimensional Regularization: The Number of Dimensions as
%a Regularizing Parameter, 
{\it Nuovo Cim.}\ {\bf 12B} (1972) 20-26.

\bibitem{NPB72} G.\ 't Hooft y M.\ Veltman,
%Regularization and Renormalization of gauge fields,
{\it Nucl.\ Phys.}\ {\bf B44} (1972) 189-213.

\bibitem{PLB72} C.G.\ Bollini y J.J. Giambiagi,
%Lowest order ``divergent'' graphs in $\nu$-dimensional space, 
{\it Phys.\ Lett.}\ {\bf 40B} (1972) 566-568.

\bibitem{FGML} H.\ Fritzsch, M.\ Gell-Mann y H.\ Leutwyler,
% ADVANTAGES OF THE COLOR OCTET GLUON PICTURE
{\it Phys.\ Lett.}\ {\bf 47B} (1973) 365-368.

\bibitem{GWP} D.J.\ Gross y F. Wilczek,
{\it Phys.\ Rev.\ Lett.}\ {\bf 30} (1973) 1343-1346.
H.D.\ Politzer, {\it Phys.\ Rev.\ Lett.}\ {\bf 30} (1973) 1346-1349.

\bibitem{ceci} C.\ Jarlskog, ``Background information
on the 1999 Nobel Prize in Physics'',\\
www.nobelprize.org/nobel$\_$prizes/physics/laureates/1999/advanced-physicsprize1999.pdf

\bibitem{velt} M.\ Veltman, 
%Nobel Lecture: From weak interactions to gravitation,
{\it Rev.\ Mod.\ Phys.} {\bf 72} (2000) 341-349.

\end{thebibliography}

